The structure of hypersonic shock waves using Navier-Stokes equations modified to include mass diffusion

Howard Brenner has recently proposed modifications to the Navier-Stokes equations that relate to a diffusion of fluid volume that would be significant for flows with high density gradients. In a previous paper (Greenshields & Reese, 2007), we found these modifications gave good predictions of the viscous structure of shock waves in argon in the range Mach 1.0-12.0 (while conventional Navier-Stokes equations are known to fail above about Mach 2). However, some areas of concern with this model were a somewhat arbitrary choice of modelling coefficient, and potentially unphysical and unstable solutions. In this paper, we therefore present slightly different modifications to include molecule mass diffusion fully in the Navier-Stokes equations. These modifications are shown to be stable and produce physical solutions to the shock problem of a quality broadly similar to those from the family of extended hydrodynamic models that includes the Burnett equations. The modifications primarily add a diffusion term to the mass conservation equation, so are at least as simple to solve as the Navier-Stokes equations; there are none of the numerical implementation problems of conventional extended hydrodynamics models, particularly in respect of boundary conditions. We recommend further investigation and testing on a number of different benchmark non-equilibrium flow cases.

==> gnuplot/Mach11Profile <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/Mach11profile.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt 0 lw 1.5 pt 2 ps 1
set style line 3 lt 4 lw 1.5 pt 3 ps 1
set style line 4 lt 2 lw 1.5 pt 3 ps 1
set style line 5 lt 1 lw 1.5 pt 3 ps 1
set style line 6 lt 3 lw 1.5 pt 3 ps 1

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 2
set nolabel
set nologscale
set key left top Left reverse samplen 2
set noarrow
set size nosquare 0.65,0.85
#set size nosquare 1.0,1.0
set nogrid

#
# Labels
#
set format x "%0.0f"
set format y "%0.1f"
set xlabel "Distance through shock [$\\lambda_{M1}$]" -0.5,0
set ylabel "Normalised density $\\rho^{\\star}$, temperature $T^{\\star}$"
set label 1 "$T^{\\star}$" at -6.0,0.3 right
set arrow 1 from -5.95,0.32 to -2.4,0.32
set arrow 2 from -5.95,0.30 to -3.6,0.30
set arrow 3 from -5.95,0.28 to -5,0.28
set label 2 "$\\rho^{\\star}$" at 3,0.8 left
set arrow 4 from 2.95,0.79 to 1.75,0.79
set arrow 5 from 2.95,0.81 to 0.95,0.81

lambda=(8.0/5.0)*sqrt(2/pi/(5.0/3.0))

plot [-10:5][-0.1:1.1] \
\
'gnuplot/Mach11rhoStarOettinger.xy' \
using (($1+0.79)/lambda):2 \
title "\\small modified N-S \\normalsize" \
with lines ls 5, \
\
'gnuplot/Mach11rhoStar.xy' \
using (($1-0.15)/lambda):2 \
title "\\small Navier-Stokes \\normalsize" \
with lines ls 4, \
\
'gnuplot/Mach11TstarOettinger.xy' \
using (($1+0.79)/lambda):2 \
notitle \
with lines ls 5, \
\
'gnuplot/Mach11Tstar.xy' \
using (($1-0.15)/lambda):2 \
notitle \
with lines ls 4, \
\
'gnuplot/Mach11_DSMC_Density.txt' \
using (($1+0.04)):((1.542824371218E0+$2)/(7.248255726316E-1+1.542824371218E0)) \
title "\\small DSMC \\normalsize" \
with points ls 1, \
\
'gnuplot/Mach11_DSMC_Temperature.txt' \
using (($1+0.04)):((1.484062774330E0+$2)/(7.838165709920E-1+1.484062774330E0)) \
notitle \
with points ls 1

#'standingShockMach8/180/rho.xy' using ($1-0.69):(($2-1.67)/4.67) \
#title "Brenner-Newton-Fourier, no volume diffusion work" \
#with lines ls 4, \
#'standingShockMach8Brenner/80/rho.xy' using ($1-0.955):(($2-1.67)/4.67) \
#title "Newton-Brenner s = 0.68" \
#with lines ls 4, \
#'standingShockMach8Brenner/240/rho.xy' using ($1-1.345):(($2-1.67)/4.67) \
#title "Newton-Brenner s = 0.76" \
#with lines ls 6, \

#
# Reset output and terminal
#
set output
set term x11



==> gnuplot/Mach9Profile <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/Mach9profile.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt 0 lw 1.5 pt 2 ps 1
set style line 3 lt 4 lw 1.5 pt 3 ps 1
set style line 4 lt 2 lw 1.5 pt 3 ps 1
set style line 5 lt 1 lw 1.5 pt 3 ps 1
set style line 6 lt 3 lw 1.5 pt 3 ps 1

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 2
set nolabel
set nologscale
#set key left top Left reverse samplen 2
set key right bottom Right noreverse samplen 2
set noarrow
set size nosquare 0.65,0.85
set nogrid

#
# Labels
#
set format x "%0.0f"
set format y "%0.1f"
set xlabel "Distance through shock [$\\lambda_{M1}$]" -0.5,0
set ylabel "Normalised density $\\rho^{\\star}$, temperature $T^{\\star}$"
set label 1 "$T^{\\star}$" at -1.5,0.8 right
#set arrow 1 from -1.45,0.81 to -0.65,0.81
#set arrow 2 from -1.45,0.80 to -0.35,0.80
set arrow 2 from -1.45,0.79 to -0.60,0.79
set arrow 3 from -1.45,0.81 to -0.05,0.81
set label 2 "$\\rho^{\\star}$" at 2.3,0.8 left
set arrow 4 from 2.25,0.79 to 1.50,0.79
set arrow 5 from 2.25,0.81 to 0.90,0.81
set label 3 "(b)" at -5.5,1.0 left

lambda=(8.0/5.0)*sqrt(2/pi/(5.0/3.0))

plot [-6:6][-0.1:1.1] \
\
'gnuplot/Mach9rhoStarOettinger.xy' \
using (($1+1.00)/lambda):2 \
title "\\small modified N-S \\normalsize" \
with lines ls 5, \
\
'gnuplot/Mach9rhoStar.xy' \
using (($1-0.12)/lambda):2 \
title "\\small Navier-Stokes \\normalsize" \
with lines ls 4, \
\
'gnuplot/Mach9TstarOettinger.xy' \
using (($1+1.00)/lambda):2 \
notitle \
with lines ls 5, \
\
'gnuplot/Mach9Tstar.xy' \
using (($1-0.12)/lambda):2 \
notitle \
with lines ls 4, \
\
'gnuplot/Argon_Mach9_density_vs_mfp.txt' \
title "\\small Experiment \\normalsize" \
with points ls 1

#\
#'../JFMresults/standingShockMach9Brenner/100/Tstar.xy' \
#using (($1+0.25)/lambda):2 \
#notitle \
#with lines ls 4, \
#\
#\
#'../JFMresults/standingShockMach9Brenner/100/rhoStar.xy' \
#using (($1+0.25)/lambda):2 \
#title "\\small Brenner-Navier-Stokes \\normalsize" \
#with lines ls 4, \
#
# Reset output and terminal
#
set output
set term x11


==> gnuplot/MachVsAsymmetryQuotient <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/MachVsAsymmetryQuotient.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt 0 lw 1.5 pt 2 ps 1
set style line 3 lt 4 lw 1.5 pt 3 ps 1
set style line 4 lt 2 lw 1.5 pt 3 ps 1
set style line 5 lt 1 lw 1.5 pt 3 ps 1
set style line 6 lt 3 lw 1.5 pt 3 ps 1

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 1
set nolabel
set nologscale
set key 2.0,1.54 Left reverse samplen 2 nobox

#
set noarrow
set size nosquare 0.8,1.0
set nogrid

#
# Labels
#
set format x "%0.0f"
set format y "%0.1f"
set xlabel "Mach number" 0,0
set ylabel "Asymmetry quotient, $Q_{\\rho}$"
#set label 1 "\\small Navier-Stokes\\normalsize" at 9.3,1.42 right
#set label 2 "\\small Brenner-Navier-Stokes\\normalsize" at 9.3,0.97 right
#set label 3 "\\small Experiment\\normalsize" at 9.3,1.18 right

plot [1:9.5][0.8:1.6] \
'gnuplot/Argon_Qrho_simulation' using ($1):($4) \
smooth csplines ls 5 \
title "\\small modified N-S\\normalsize", \
'gnuplot/Argon_Qrho_simulation' using ($1):($2) \
smooth csplines ls 4 \
title "\\small Navier-Stokes\\normalsize", \
'gnuplot/arq.dat' \
title "\\small Experiment\\normalsize" \
with points ls 1

#show label 1
#show label 2
#show label 3

#
# Reset output and terminal
#
set output
set term x11


==> gnuplot/MachVsAsymmetryQuotientSmall <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/MachVsAsymmetryQuotient.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt 0 lw 1.5 pt 2 ps 1
set style line 3 lt 4 lw 1.5 pt 3 ps 1
set style line 4 lt 2 lw 1.5 pt 3 ps 1
set style line 5 lt 1 lw 1.5 pt 3 ps 1
set style line 6 lt 3 lw 1.5 pt 3 ps 1

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 1
set nolabel
set nologscale
#set key 2.0,1.54 Left reverse samplen 2 nobox
set key right bottom Right noreverse samplen 2 spacing 0.8
#
set noarrow
set size nosquare 0.65,0.85
#set size nosquare 0.8,1.0
set nogrid

#
# Labels
#
set format x "%0.0f"
set format y "%0.1f"
set xlabel "Mach number" 0,0
set ylabel "Asymmetry quotient, $Q_{\\rho}$"
#set label 1 "\\small Navier-Stokes\\normalsize" at 9.3,1.42 right
#set label 2 "\\small Brenner-Navier-Stokes\\normalsize" at 9.3,0.97 right
#set label 3 "\\small Experiment\\normalsize" at 9.3,1.18 right

plot [1:9.5][0.8:1.6] \
'gnuplot/Argon_Qrho_simulation' using ($1):($4) \
smooth csplines ls 5 \
title "\\small modified N-S\\normalsize", \
'gnuplot/Argon_Qrho_simulation' using ($1):($2) \
smooth csplines ls 4 \
title "\\small Navier-Stokes\\normalsize", \
'gnuplot/arq.dat' \
title "\\small Experiment\\normalsize" \
with points ls 1

#show label 1
#show label 2
#show label 3

#
# Reset output and terminal
#
set output
set term x11


==> gnuplot/MachVsInvDensThickness <==
#set term dumb 45 15
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/MachVsInvShockThickness.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt 0 lw 1.5 pt 2 ps 1
set style line 3 lt 4 lw 1.5 pt 3 ps 1
set style line 4 lt 2 lw 1.5 pt 3 ps 1
set style line 5 lt 1 lw 1.5 pt 3 ps 1
set style line 6 lt 3 lw 1.5 pt 3 ps 1

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 1
#set label 1 "\\small $0.68$\\normalsize" at 11.1,0.267 left
#set label 2 "\\small $0.72$\\normalsize" at 11.1,0.230 left
#set label 3 "\\small $0.76$\\normalsize" at 11.1,0.200 left
#set label 4 "\\small $s =$\\normalsize" at 11.1,0.297 left
set nologscale
set key 4.5,0.15 Left reverse samplen 2
#set key below Left reverse
set nolabel
set noarrow
set size nosquare 0.8,1.0
set nogrid

#
# Labels
#
set format x "%0.0f"
set format y "%0.2f"
set xlabel "Mach number" 0,0
set ylabel "Inverse density thickness, $L_{\\rho}^{-1}$"

lambda=(8.0/5.0)*sqrt(2/pi/(5.0/3.0))

plot [1:11][0.05:0.5] \
\
'gnuplot/Argon_IDT_simulation' using ($1):(lambda*$4) \
smooth csplines ls 5 \
title "\\small modified N-S\\normalsize", \
\
'gnuplot/Argon_IDT_simulation' using ($1):(lambda*$2) \
smooth csplines ls 4 \
title "\\small Navier-Stokes\\normalsize", \
\
'gnuplot/Argon_idt_vs_MachNo.txt' \
title "\\small Experiment\\normalsize" \
with points ls 1

#show label 1
#show label 2
#show label 3
#show label 4

#'Argon_idt_Simulations' using ($1):($3) \
#smooth csplines ls 3 \
#title "Newton-Brenner s = 0.76, no volume diffusion work", \
#
# Reset output and terminal
#
set output
set term x11


#'Argon_idt_Simulations' using ($1):($2) smooth csplines title "Newtonian - $\\U_{m}$", \
#'Argon_idt_Simulations' using ($1):($3) smooth csplines title "Newtonian - $\\U_{v}$ (Brenner)"


==> gnuplot/spatialStabilityPlot <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/SpatialStabilityOettingerNoBlock.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt -1 lw 1.5 pt 2 ps 1
set style line 3 lt 0 lw 1.5 pt 2 ps 1
set style line 4 lt 4 lw 1.5 pt 3 ps 1
set style line 5 lt 2 lw 1.5 pt 3 ps 1
set style line 6 lt 1 lw 1.5 pt 3 ps 1
set style line 7 lt 3 lw 1.5 pt 3 ps 1
set style data lines

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 1
set nolabel
set nologscale
set nokey
#set key 0.7,2.5 Left reverse samplen 2
set key default top samplen 2
set noarrow
set size nosquare 0.65,0.85
set nogrid

set format x "%0.0f"
set format y "%0.0f"
set xlabel "Wave number, $k_{r}$"
set ylabel "Attenuation constant, $k_{i}$" 0.5,0.0
set arrow 1 from -3,0 to 3,0 nohead ls 1
set arrow 2 from 0,-3 to 0,3 nohead ls 1
set arrow 3 from -2.25,2.0 to -2.35,2.1 head size 0.8,15 filled ls 2
set arrow 4 from  2.25,-2.0 to  2.35,-2.1 head size 0.8,15 filled ls 2
set arrow 5 from -2.05,2.0 to -2.15,2.1 head size 0.8,15 filled ls 2
set arrow 6 from  2.05,-2.0 to  2.15,-2.1 head size 0.8,15 filled ls 2
set arrow 7 from -1.5,2.0 to -1.6,2.1 head size 0.8,15 filled ls 2
set arrow 8 from  1.5,-2.0 to  1.6,-2.1 head size 0.8,15 filled ls 2
set arrow 9 from -1.0,1.26 to -1.1,1.36 head size 0.8,15 filled ls 2
set arrow 10 from  1.0,-1.26 to  1.1,-1.36 head size 0.8,15 filled ls 2
set label 1 "(b)" at -2.7,-2.6

set style data points
plot [-3:3] [-3:3] \
'gnuplot/spatialAlpha1.0' using 2:3 title "\\small $\\Sc = 1.0$\\normalsize" with lines ls 2, \
'gnuplot/spatialAlpha1.0' using 4:5 notitle with lines ls 2, \
'gnuplot/spatialAlpha1.0' using 6:7 notitle with lines ls 2, \
'gnuplot/spatialAlpha1.0' using (-$2):(-$3) notitle with lines ls 2, \
'gnuplot/spatialAlpha1.0' using (-$4):(-$5) notitle with lines ls 2, \
'gnuplot/spatialAlpha1.0' using (-$6):(-$7) notitle with lines ls 2, \
'gnuplot/spatialAlpha5.0' using 2:3 title "\\small $\\Sc = 0.2$\\normalsize" with lines ls 3, \
'gnuplot/spatialAlpha5.0' using 4:5 notitle with lines ls 3, \
'gnuplot/spatialAlpha5.0' using 6:7 notitle with lines ls 3, \
'gnuplot/spatialAlpha5.0' using (-$2):(-$3) notitle with lines ls 3, \
'gnuplot/spatialAlpha5.0' using (-$4):(-$5) notitle with lines ls 3, \
'gnuplot/spatialAlpha5.0' using (-$6):(-$7) notitle with lines ls 3
#'alpha0.0' using 4:5 title "\\small Navier-Stokes\\normalsize" with lines ls 3, \
#'alpha0.0' using 6:7 notitle with lines ls 3, \
#'alpha0.0' using (-$4):(-$5) notitle with lines ls 3, \
#'alpha0.0' using (-$6):(-$7) notitle with lines ls 3

#-5 with boxes, \
#0 with filledcurve y1=-10 fs solid 0.25 lt 8, \
#
# Reset output and terminal
#
set output
set term x11



==> gnuplot/temporalStabilityPlot <==
#set term x11
set term epslatex default monochrome dashed "default" 12
set output "figures/TemporalStabilityOettingerNoBlock.eps"
#
# Define linestyles
#
set style line 1 lt -1 lw 1 pt 2 ps 1
set style line 2 lt -1 lw 1.5 pt 2 ps 1
set style line 3 lt 0 lw 1.5 pt 2 ps 1
set style line 4 lt 4 lw 1.5 pt 3 ps 1
set style line 5 lt 2 lw 1.5 pt 3 ps 1
set style line 6 lt 1 lw 1.5 pt 3 ps 1
set style line 7 lt 3 lw 1.5 pt 3 ps 1
set style data lines

#
# Graph format
#
set ticscale 0.5
set border 31 ls 1
set nomxtics
set xtics 1
set nolabel
set nologscale
set nokey
#set key 1.0,-2.6 Left reverse samplen 2
set key default bottom samplen 2
set noarrow
set size nosquare 0.65,0.85
set nogrid

set format x "%0.0f"
set format y "%0.0f"
set xlabel "Frequency dispersion, $\\omega_{r}$"
set ylabel "Frequency attenuation, $\\omega_{i}$" 0.5,0.0
set arrow 1 from 0,10 to 0,-5 nohead ls 1
set arrow 2 from 3,0 to -3,0 nohead ls 1
set arrow 3 from 0,7.8 to 0,8 head size 0.8,15 filled ls 2
set arrow 5 from 2.03,6 to 2.06,6.2 head size 0.8,15 filled ls 2
set arrow 6 from -2.03,6 to -2.06,6.2 head size 0.8,15 filled ls 2
set arrow 7 from 0.75,2.7 to 0.75,2.9 head size 0.8,15 filled ls 2
set arrow 8 from -0.75,2.7 to -0.75,2.9 head size 0.8,15 filled ls 2
set label 1 "(a)" at -2.7,-3.9

set style data points
plot [-3:3] [-5:10] \
'gnuplot/temporalAlpha1.0' using 2:3 \
title "\\small $\\Sc = 1.0$\\normalsize" with lines ls 2, \
'gnuplot/temporalAlpha1.0' using 4:5 notitle with lines ls 2, \
'gnuplot/temporalAlpha1.0' using 6:7 notitle with lines ls 2, \
'gnuplot/temporalAlpha5.0' using (-$4):5 \
title "\\small $\\Sc = 0.2$\\normalsize" with lines ls 3, \
'gnuplot/temporalAlpha5.0' using 4:5 notitle with lines ls 3, \
'gnuplot/temporalAlpha5.0' using 6:7 notitle with lines ls 3
#'alpha0.0' using 2:3 title "\\small Navier-Stokes\\normalsize" with lines ls 3, \
#'alpha0.0' using 4:5 notitle with lines ls 3, \
#'alpha0.0' using 6:7 notitle with lines ls 3

#-5 with boxes, \
#0 with filledcurve y1=-10 fs solid 0.25 lt 8, \
#
# Reset output and terminal
#
set output
set term x11


